Gate-Voltage Tunability of Plasmons in Single and Multi-layer Graphene Structures: Analytical Description and Concepts for Terahertz Devices

The strong light-matter interaction in graphene over a broad frequency range has opened up a plethora of photonics applications of graphene. The goal of this paper is to present the voltage tunability of plasmons in gated single- and multi-layer graphene structures. Device concepts for plasmonic interconnects and antennas and their performance for THz communication are presented. For the first time, the role of gate voltage and the thickness of the gate dielectric on the characteristics of plasmon propagation in graphene are quantified by accounting for both the interface trap capacitance and the quantum capacitance. The gate voltage serves as a powerful knob to tweak the carrier concentration and allows building electrically reconfigurable terahertz devices. By optimizing the gate voltage to maximize the plasmon propagation length in a gated multi-layer graphene geometry, we derive simple scaling trends that give intuitive insight into device modeling and design.

==> Abstract.tex <==
\begin{abstract}
The strong light-matter interaction in graphene over a broad frequency range has opened up a plethora of photonics applications of graphene. The goal of this paper is to present the voltage tunability of plasmons in gated single- and multi-layer graphene structures. Device concepts for plasmonic interconnects and antennas and their performance for THz communication are presented. For the first time, the role of gate voltage and the thickness of the gate dielectric on the characteristics of plasmon propagation in graphene are quantified by accounting for both the interface trap capacitance and the quantum capacitance. The gate voltage serves as a powerful knob to tweak the carrier concentration and allows building electrically reconfigurable terahertz devices. By optimizing the gate voltage to maximize the plasmon propagation length in a gated multi-layer graphene geometry, we derive simple scaling trends that give intuitive insight into device modeling and design. 
\end{abstract}

%\begin{IEEEkeywords}
Keywords - Single- and multi-layer graphene, plasmons, interface states, terahertz communication, antenna
%\end{IEEEkeywords}


==> preamble.tex <==
%
\title{Gate-Voltage Tunability of Plasmons in Single- and Multi-layer Graphene Structures \textendash {Analytical} Description and Concepts for Terahertz Devices}
%
\author{Shaloo~Rakheja,~\IEEEmembership{Member,~IEEE},
        and~Parijat~Sengupta%
\thanks{S. Rakheja is with the department of Electrical and Computer Engineering, New York University, Brooklyn NY 11201 (email: shaloo.rakheja@nyu.edu). P. Sengupta is with the Photonics Center, Boston University, Boston, MA, 02215.}}% 
%\thanks{This work was sponsored by NSF NEEDS program.}}
% The paper headers
\markboth{IEEE Transactions on Nanotechnology- Draft Copy}%~Vol.~21, No.~2, January~2010}%
{Shell \MakeLowercase{\textit{et al.}}: Bare Demo of IEEEtran.cls for Journals}	
